Synthesis from Satisficing and Temporal Goals

Reactive synthesis from high-level specifications that combine hard constraints expressed in Linear Temporal Logic LTL with soft constraints expressed by discounted-sum (DS) rewards has applications in planning and reinforcement learning. An existing approach combines techniques from LTL synthesis with optimization for the DS rewards but has failed to yield a sound algorithm. An alternative approach combining LTL synthesis with satisficing DS rewards (rewards that achieve a threshold) is sound and complete for integer discount factors, but, in practice, a fractional discount factor is desired. This work extends the existing satisficing approach, presenting the first sound algorithm for synthesis from LTL and DS rewards with fractional discount factors. The utility of our algorithm is demonstrated on robotic planning domains.

==> Section/prelims.tex <==
\section{Preliminaries}
\label{Sec:Prelims}


\subsection{Linear Temporal Logic}

{Linear Temporal Logic} ($\ltl$) extends propositional logic with infinite-horizon temporal operators. The syntax of an $\ltl$ is defined as $\varphi:= a \in \ap \mid \ltlNeg \varphi \mid \varphi \land \varphi \mid \varphi \lor \varphi \mid \ltlX \varphi \mid \varphi \ltlU \varphi \mid \ltlF \varphi \mid \ltlG \varphi$. 
Here $\ltlX$ (Next), $\ltlU$ (Until), $\ltlF$ (Eventually), $\ltlG$ (Always) are temporal operators.  
The semantics of $\ltl$ can be found in~\cite{pnueli1977temporal}. 
%The language of an $\ltl$ formula $\varphi$, denoted by $\L(\varphi)$, is the set of finite words over $2^{\ap}$  that satisfy $\varphi$.



\subsection{B\"uchi Automata and Co-safety Automata}

A B\"uchi automaton~\cite{thomas2002automata} is a tuple
  $\A = (\Statess$, $\Sigma$, $\delta$, $s_\mathcal{I}$, $\Final)$, where
  $ \Statess $ is a finite set of states, $ \Sigma $ is a finite input alphabet,  $ \delta \subseteq (\Statess \times \Sigma \times \Statess) $ is the transition relation, state $ s_\mathcal{I} \in \Statess $ is the initial state, and $ \Final \subseteq \Statess $ is the set of  accepting states.
A B\"uchi automaton is  deterministic if for all states $ s $ and
inputs $a$, $ |\{s'|(s, a, s') \in \delta \textrm{ for some $s'$} \}|
= 1 $.
We use the standard semantics of a B\"uchi automaton~\cite{thomas2002automata} (Details in appendix). %For a word $ w = w_0w_1\dots \in \Sigma^{\omega} $, a run $ \rho$ of $ w $ is a sequence of states $s_0s_1\dots$ s.t.$ s_0 = s_\mathcal{I}$, and $ \tau_i =(s_i, w_i, s_{i+1}) \in \delta $ for all $i$.Let $ \mathit{inf}(\rho) $ denote the set of states that occur infinitely often in run ${\rho}$. A run $\rho$ is an accepting run if $ \mathit{inf}(\rho)\cap \Final \neq \emptyset $. A word $w$ is an accepting word if it has an accepting run. The language of B\"uchi automaton $\A$ is the set of all words accepted by $\A$. Languages accepted by B\"uchi automata are called  $\omega$-regular.

A co-safety automaton~\cite{kupferman1999model} is a deterministic B\"uchi automaton containing a single accepting state. All outgoing transitions from this state loop back to it. Thus, this state is called an \emph{accepting sink}. %Thus, every accepting word must have a finite-prefix which visits the accepting sink.

\subsection{Graph Games}

A (two-player) graph game is defined over the structure  $G = (V  = V_s \uplus V_e, \init, E, \alpha)$~\cite{thomas2002automata}.
It consists of a directed graph $(V,E)$,
and a partition $(V_s, V_e)$ of its  states $V$ belonging to the system player $P_s$ and the environment player $P_e$, respectively. 
State $\init$ is the initial state. 
$vE $ designates the set of successors of state $v$. For convenience, we assume that every state has at least one outgoing edge, i.e, $vE  \neq \emptyset$ for all $v \in V$.

A play is an infinite path created by the  players moving a token along the transitions as follows:
The token is at the initial state in the start. If the current
position $v$ belongs to $V_i$, then $P_i$ chooses the successor state from $vE$, for $i \in\{e,s\}$.
Formally, a play $\rho = v_0v_1v_2\dots$ is an infinite sequence of states such that  $v_0 = v_{\mathsf{init}}$, and each pair of successive states is a transition, i.e., $(v_k, v_{k+1}) \in E$ for all $k\geq 0$. 

The winning condition is determined by $\alpha$: (a). When $\alpha$ is a set $\F\subseteq V$ of states, the graph game is called a \emph{reachability} game. A play is winning for the system if it visits a state in $\F$, and winning for the environment otherwise. 
(b). When  $\alpha$ is a {\em coloring function} $c:V\rightarrow \N$, which assigns a natural-valued {\em color} to states in the game, the game is called a \emph{parity game} \cite{jurdzinski1998deciding}.
A {\em color sequence} of a play $c_\rho = c(v_0)c(v_1)c(v_2)\ldots$. A play is winning for the system if the maximum color appearing infinitely often in its color sequence is even, and winning for the environment otherwise \cite{jurdzinski1998deciding}.  


A {\em strategy} for a player guides the player on which state to go to next based on the history of the play. Formally, a strategy for $P_i$ is a function 
$\sigma_i:V^*V_i \rightarrow V$ for $i \in \{s,e\}$. A strategy if winning for a player in a graph game if it guarantees that all resulting plays are winning for the player.

To solve a graph game is to determine if the system has a winning strategy. Standard results show that reactive synthesis from specifications represented by co-safety automata and (non-deterministic) B\"uchi automata reduces to solving a reachability game and a parity game, resp.~\cite{thomas2002automata}. 




==> Section/tables.tex <==

\input{Table/Grid4}

\input{Table/Grid6}

\input{Table/Grid8}
\input{Table/Grid10}

\input{Table/conveyor_3_5}
\input{Table/conveyor_3_6}
\input{Table/conveyor_3_8}
\input{Table/conveyor_3_10}
\input{Table/conveyor_4_5}
\input{Table/conveyor_4_6}
\input{Table/conveyor_4_8}
\input{Table/conveyor_4_10}




==> test.tex <==

\section{IJCAI Rebuttal}

We thank the reviewers for their helpful suggestions and comments. We will incorporate them into the paper. 
If accepted, we will purchase an extra page to incorporate the suggestions and comments. 


\subsection*{Reviewer 66: Clarity of Theorem 2}

We agree with the reviewer that adding an example will enhance the readability of Theorem 2. In the final version, we will demonstrate how a comparator accepts and rejects weight-sequences through examples. 

In some more detail, Theorem 2 states that with an approximation factor, we need to only consider a finite history of a weight-sequence to ensure that its discounted-sum exceeds our threshold.
To make this point, we will illustrate how the weight-sequence $A = -1, 0, 1^\omega$ is accepted by a comparator with discount factor $d = 1.5$ i.e. $(1+2^{-1})$ and approximation factor $\varepsilon=0.5$ i.e. $(2^{-1})$ when the 
threshold value is $\nu = 0$, relation $R$ is $\geq$, and upper bound is $\mu = 1$. 
We will also explain how weight-sequence $B = -1,-1,1^{\omega}$ is rejected by the same comparator. A portion of the comparator needed to illustrate these two points has been presented in ~\autoref{Fig:comparator}. 


\begin{figure}[h]
\caption{Portion of comparator to illustrate the acceptance of $A = -1,0,1^\omega$ and rejection of $B=-1,-1,1^{\omega}$}
\label{Fig:comparator}
\centering
\begin{tikzpicture}[->,auto,node distance=1.8cm,on grid,line width=0.4mm]
          \tikzstyle{round}=[thick,draw=black,circle]
          
  \node[state,initial] (0) {$0$};
  \node[state] (-4) [right of=0] {$-4$};
  \node[state, accepting] (10) [right of=-4] {$10$};
  %\node[state,accepting] ($10$) [right of=10] {$A$};
  \node[state] (-6) [above left of=-4] {$-6$};
  \node[state] (-5) [right of=-6] {$-5$};
  \node[state] (-8) [below right of=-4] {$-8$};

  \path (0) edge                node {$-1$} (-4)
        (-4) edge               node {$1$} (10)
        (10) edge [loop right]  node {$*$} (10)
        (-4) edge [above]       node {$0$} (-6)
        (-6) edge               node {$1$} (-5)
        (-5) edge               node {$1$} (-4)
        (-4) edge  [above]      node {$-1$} (-8)
        %(A) edge [loop above]  node {$*$} (A)
        (-8) edge [loop right]  node {$*$} (-8);

\end{tikzpicture}
\end{figure}


\subsection*{Reviewers 81 and 93: Experiments}

\paragraph{Both.}

The reviewers have asked for a broader experimental coverage. While we would always like to include more diverse experiments, space constraints force us to make trade offs. We  settled on two sets of experiments. The first, based on a typical gridworld, is chosen because we expect it to be the most familiar to our readers. The second is chosen because of its relevance to robotics. These experiments were inspired by a manipulation domain. %introduced in a recent robotics paper. 
We will clarify the relevance to robotics in the final draft.



\paragraph{Reviewer 93.}
First, we would like to thank the reviewer for pointing out that we didn't present experiments varying the approximation factor. This was a major oversight and will be included in the final draft of the paper. Please see \autoref{table:approx_factor}.

We would like to clarify that the experiments in Figure 2 vary both the positive reward and the discount factor. We will redo this figure to separate the two to improve legibility.
% So, Figure 2 also shows how the algorithm scales with the positive reward. 

The suggestion for the symbolic algorithm is an excellent one, but we see it as a future direction. Although the comparator is an automaton, their transitions are associated with a (quantitative) semantic meaning. We would, thus, like to thoroughly explore symbolic representations of  comparators before designing symbolic algorithms with them.

We expect the approach with integer discount factors to be faster on an identical game (same rewards) since it has lower complexity. Since, however, the quality of solution would be  poor in this case, this would not present a fair comparison. 
%\input{IJCAIRebuttal/approx_test}


\subsection*{Reviewer 93: On the need of fractional dis. factors}
As we understand it, the reviewer's concerns can be posed as the following question:
{\em Are there scenarios where non-integer discount factors are needed or can all scenarios be ``simulated'' by scaling appropriate integer rewards and integer discount factors?}
This is a good question. Unfortunately, it is not known how to perform such scaling. Note that such scaling would possibly provide a solution to Discounted-sum inclusion under non-integer discount factors - an important open problem for which even decidability is currently unknown [Chatterjee, Doyen, Henzinger; ACM ToCL 2010]. 

Even then, if we use integer discount factors with scaled rewards, the rewards would have to be scaled up by a very large value. This would  make problem specification non-intuitive since the rewards would be tailored to the discount factor. In our experience, this was not the case with fractional discount factors: Even un-tailored rewards  generated high-quality solutions. We will include a detailed discussion in paper. 



\section{Individual Comments}

\paragraph{R39} We will include a definition of LTL in the main paper. 

\paragraph{R66}
The human and robot can interfere by blocking each others motions in the domain introduced in a recent ICRA paper. We will cite the paper in the final version.

